Hierarchical Policy Learning via Spectral Decomposition

In this paper, we identify a semantic decomposition in robot action sequences, separating task-level motion intent from execution-level refinements. By analyzing actions in the spectral domain using the discrete cosine transform (DCT), we observe that low-frequency components capture global motion trajectories, while high-frequency components encode precise timing, alignment, and contact behaviors. Motivated by this structure, we propose Causal Spectral Policy (CSP), which models action generation as a causal coarse-to-fine process: coarse motion is predicted from observation and language, and fine corrections are generated conditionally on the realized trajectory. Across simulation and real-world evaluations, CSP consistently outperforms strong baselines on precision-sensitive manipulation tasks. Additionally, we propose human-inspired teleoperation noise injection as a data augmentation method, under which our approach demonstrates strong robustness to noisy demonstrations.

==> sections/4_method_old.tex <==
\section{Method}

Our method models action generation as a coarse-to-fine process over temporal scales. For each action chunk $a_{t:t+K-1}$, we first transform the action sequence into the temporal frequency domain using the discrete cosine transform (DCT), and define low- and high-frequency components by partitioning the resulting coefficients. The action can then be written as
\[
a_{t:t+K-1} = a^{\mathrm{low}}_{t:t+K-1} + a^{\mathrm{high}}_{t:t+K-1},
\]
where the low-frequency component captures smooth, slowly varying motion that determines overall task progress, and the high-frequency component captures short-timescale variations related to precise alignment and contact.

Based on this decomposition, we model action generation causally. The low-frequency component is predicted from the observation and language instruction, $a^{\mathrm{low}} \sim \pi^{\mathrm{low}}_\theta(o_t, l)$, while the high-frequency component is predicted conditionally on the realized coarse motion, $a^{\mathrm{high}} \sim \pi^{\mathrm{high}}_\theta(o_t, a^{\mathrm{low}})$. This structure separates task-level intent from execution-level refinement and enables more robust learning under noisy demonstrations.


\subsection{Action Representation: Spectral Domain}

We represent each action chunk $a_{t:t+K-1} \in \mathbb{R}^{K \times d}$ in a temporal frequency domain using the discrete cosine transform (DCT). 
Let $F \in \mathbb{R}^{K \times K}$ denote an orthonormal DCT basis applied independently to each action dimension. 
The coefficient representation is
\[
c_t = F a_{t:t+K-1}, \qquad a_{t:t+K-1} = F^{-1} c_t .
\]

Because $F$ is orthonormal, this transformation preserves Euclidean distance:
\[
\| \hat a_{t:t+K-1} - a_{t:t+K-1} \|_2^2
=
\| \hat c_t - c_t \|_2^2 .
\]
Thus, learning in the spectral domain does not approximate or distort the original action sequence, but provides an equivalent reparameterization in which temporal structure is made explicit.

A key benefit of this representation is that it exposes heterogeneity across temporal scales.
Empirically, manipulation trajectories exhibit strong energy concentration in low-frequency coefficients, while high-frequency coefficients have smaller magnitude and are more sensitive to execution noise.
This structure is difficult to isolate in the time domain, where all timesteps are treated symmetrically.

To formalize this, consider a noisy demonstration
\[
\tilde a_{t:t+K-1} = a_{t:t+K-1} + \varepsilon,
\]
with corresponding spectral coefficients
\[
\tilde c_t = F \tilde a_{t:t+K-1} = c_t + \eta,
\qquad \eta = F \varepsilon .
\]
Human teleoperation noise is temporally correlated and concentrates on short timescales, which implies that its energy is primarily contained in high-frequency coefficients.
As a result, we have
\[
\eta^{\mathrm{low}} \approx 0, 
\qquad 
\eta^{\mathrm{high}} \text{ large}.
\]

Under a standard squared-loss objective, training a policy to regress actions from noisy demonstrations yields
\[
\mathbb{E}\!\left[\|\hat c_t - \tilde c_t\|_2^2\right]
=
\mathbb{E}\!\left[\|\hat c_t^{\mathrm{low}} - c_t^{\mathrm{low}}\|_2^2\right]
+
\mathbb{E}\!\left[\|\hat c_t^{\mathrm{high}} - (c_t^{\mathrm{high}} + \eta^{\mathrm{high}})\|_2^2\right].
\]
The loss therefore decomposes additively across temporal frequencies.

This decomposition reveals an intrinsic asymmetry in learning difficulty.
Low-frequency components are supervised by clean, low-variance targets and are well-conditioned for regression.
In contrast, high-frequency components are trained against noisy targets with large conditional variance, for which the Bayes-optimal predictor under squared loss reduces to a conditional mean,
\[
\hat c_t^{\mathrm{high}}(o_t,l)
=
\mathbb{E}[c_t^{\mathrm{high}} + \eta^{\mathrm{high}} \mid o_t,l],
\]
causing unpredictable high-frequency structure to be averaged out.

Representing actions in the spectral domain therefore makes explicit which parts of the trajectory are reliably learnable from demonstrations and which are fundamentally noise-limited.
This separation motivates treating different temporal components with distinct modeling assumptions rather than learning them jointly in a monolithic representation.


\subsection{Causal Decomposition Across Temporal Scales}

Given the spectral decomposition
\[
a_{t:t+K-1} = a^{\mathrm{low}}_{t:t+K-1} + a^{\mathrm{high}}_{t:t+K-1},
\]
we impose a causal structure on action generation by factorizing
\[
p(a_{t:t+K-1} \mid o_t, l)
=
p(a^{\mathrm{low}}_{t:t+K-1} \mid o_t, l)\;
p(a^{\mathrm{high}}_{t:t+K-1} \mid o_t, a^{\mathrm{low}}_{t:t+K-1}).
\]

This factorization reflects a simple structural assumption:  
low-frequency actions encode a coarse motion plan determined by task intent, while high-frequency actions represent execution-level refinements whose meaning is defined relative to the realized coarse trajectory.

\vspace{0.3em}
\paragraph{What changes under this factorization.}
The causal decomposition modifies the conditional prediction problem faced by the policy, particularly for the high-frequency component.

\subsubsection{Learning-Theoretic Implications}

In a joint formulation, high-frequency actions are learned by minimizing
\[
\mathbb{E}\!\left[
\| \hat a^{\mathrm{high}}(o_t,l) - a^{\mathrm{high}} \|_2^2
\right],
\]
whose Bayes-optimal predictor under squared loss is
\[
\hat a^{\mathrm{high}}(o_t,l)
=
\mathbb{E}[a^{\mathrm{high}} \mid o_t,l].
\]

This predictor marginalizes over all high-frequency behaviors compatible with the observation and task instruction.
When different coarse trajectories require different refinements, these behaviors are averaged together, causing fine-scale structure to be suppressed.

Under the proposed causal factorization, the learning objective instead becomes
\[
\mathbb{E}\!\left[
\| \hat a^{\mathrm{high}}(o_t,a^{\mathrm{low}}) - a^{\mathrm{high}} \|_2^2
\right],
\qquad
\hat a^{\mathrm{high}}(o_t,a^{\mathrm{low}})
=
\mathbb{E}[a^{\mathrm{high}} \mid o_t,a^{\mathrm{low}}].
\]

Conditioning on the realized coarse motion refines the posterior distribution,
\[
p(a^{\mathrm{high}} \mid o_t,a^{\mathrm{low}})
\;\;\text{vs.}\;\;
p(a^{\mathrm{high}} \mid o_t,l),
\]
allowing predictable refinement structure to be recovered rather than averaged out.

Importantly, this change does not approximate or modify the action signal.
The decomposition is exact, and the original trajectory is recovered as
\[
a_{t:t+K-1} = a^{\mathrm{low}}_{t:t+K-1} + a^{\mathrm{high}}_{t:t+K-1}.
\]
Instead, the factorization constrains how information flows during learning, aligning the regression targets with the underlying temporal dependencies of physical manipulation.

\subsubsection{Relation to Autoregressive and Joint Sequence Prediction}

Different policy formulations correspond to different factorizations of the conditional distribution
$p(a_{t:t+K-1} \mid o_t, l)$, which in turn define different learning objectives.

Autoregressive policies factorize this distribution temporally,
\[
p(a_{t:t+K-1} \mid o_t,l)
=
\prod_{k=0}^{K-1} p(a_{t+k} \mid o_{t+k}, l),
\]
reducing learning to a sequence of local conditional predictions.

Joint sequence prediction instead learns the marginal conditional expectation
\[
\mathbb{E}[a_{t:t+K-1} \mid o_t,l],
\]
in which all intermediate temporal structure is implicitly marginalized.

In contrast, the proposed coarse-to-fine factorization
\[
p(a_{t:t+K-1} \mid o_t,l)
=
p(a^{\mathrm{low}} \mid o_t,l)\;
p(a^{\mathrm{high}} \mid o_t,a^{\mathrm{low}})
\]
introduces an explicit intermediate variable corresponding to coarse temporal structure.
This changes the statistical object being learned, replacing marginal prediction of fine-scale behavior with conditional prediction given the realized coarse trajectory.


\subsection{Learning Under Noisy Demonstrations}
\label{sec:noisy_learning}

\paragraph{Why noise is essential.}
Under clean demonstrations, different imitation learners can appear similar because supervision provides reliable targets for both slow and fast action variations. Real teleoperation data, however, contains structured execution noise that concentrates on short-timescale fluctuations. Injecting human-like noise into simulator demonstrations therefore serves as a controlled way to reveal whether a learner can recover the task-critical fast variations when they are no longer cleanly observable.

\paragraph{A simple frequency-domain model.}
Consider an action chunk $a \in \mathbb{R}^{K \times d}$ and its temporal-basis coefficients $c = F a$, where $F \in \mathbb{R}^{K\times K}$ is an orthonormal temporal transform (DCT in practice). We decompose coefficients into low- and high-frequency blocks:
\begin{equation}
c = \begin{bmatrix} c^{\mathrm{low}} \\ c^{\mathrm{high}} \end{bmatrix}, 
\qquad 
a = F^{-1} c = F^{-1}\!\begin{bmatrix} c^{\mathrm{low}} \\ c^{\mathrm{high}} \end{bmatrix}.
\end{equation}
We model a noisy demonstration as
\begin{equation}
\tilde a = a + \epsilon,
\qquad
\tilde c = F\tilde a = c + \eta,
\end{equation}
where $\eta := F\epsilon$ are the noise coefficients. Human-like noise (temporally correlated drift + sparse corrective bursts) has most of its power at short timescales; we therefore assume
\begin{equation}
\eta^{\mathrm{low}} \approx 0, 
\qquad 
\eta^{\mathrm{high}} \sim \text{large},
\label{eq:noise_high}
\end{equation}
i.e., the corruption is concentrated in the high-frequency block.

\paragraph{Why monolithic action regression fails under high-frequency noise.}
A standard chunk policy $\Pi_\theta(o,x)$ is trained by regression on the noisy targets:
\begin{equation}
\min_\theta~\mathbb{E}\big[\|\Pi_\theta(o,x)-\tilde a\|^2\big]
=
\min_\theta~\mathbb{E}\big[\|F\Pi_\theta(o,x)-\tilde c\|^2\big].
\end{equation}
Define the model prediction in coefficient space $\hat c_\theta := F\Pi_\theta(o,x)$. Because $F$ is orthonormal, the loss decomposes additively across frequency blocks:
\begin{equation}
\mathbb{E}\big[\|\hat c_\theta-\tilde c\|^2\big]
=
\mathbb{E}\big[\|\hat c_\theta^{\mathrm{low}}-c^{\mathrm{low}}\|^2\big]
+
\mathbb{E}\big[\|\hat c_\theta^{\mathrm{high}}-(c^{\mathrm{high}}+\eta^{\mathrm{high}})\|^2\big].
\label{eq:loss_split}
\end{equation}
The key issue is that the second term forces the learner to fit a \emph{noisy} target $c^{\mathrm{high}}+\eta^{\mathrm{high}}$. Even with unlimited capacity, the optimal predictor under squared loss satisfies
\begin{equation}
\hat c^{\mathrm{high}}_\star(o,x) = \mathbb{E}[c^{\mathrm{high}}+\eta^{\mathrm{high}} \mid o,x]
= \mathbb{E}[c^{\mathrm{high}}\mid o,x] + \underbrace{\mathbb{E}[\eta^{\mathrm{high}}\mid o,x]}_{\approx 0},
\end{equation}
so the best achievable solution averages out the stochastic high-frequency component. When $\mathrm{Var}(\eta^{\mathrm{high}})$ is large relative to $\mathrm{Var}(c^{\mathrm{high}} \mid o,x)$, gradients from the high-frequency block become high-variance and uninformative, and optimization is dominated by the low-frequency block. As a result, the learned policy reproduces smooth, task-progress motion but systematically misses timing-sensitive corrective behavior.

\paragraph{Why our causal decomposition helps.}
Our model explicitly factorizes action generation across temporal scales:
\begin{equation}
p(c^{\mathrm{low}}, c^{\mathrm{high}} \mid o,x)
=
p(c^{\mathrm{low}} \mid o,x)\;
p(c^{\mathrm{high}} \mid o, c^{\mathrm{low}}),
\label{eq:factorization}
\end{equation}
implemented by two predictors
\begin{equation}
\hat c^{\mathrm{low}} = f_\theta(o,x), 
\qquad
\hat c^{\mathrm{high}} = g_\phi(o, \hat c^{\mathrm{low}}),
\end{equation}
with reconstruction $\hat a = F^{-1}[\hat c^{\mathrm{low}};\hat c^{\mathrm{high}}]$.
This structure provides a stable reference for learning high-frequency behavior: conditioning on $\hat c^{\mathrm{low}}$ removes ambiguity about where the trajectory is going, so $g_\phi$ only needs to model local corrections. Under the noise model in~\eqref{eq:noise_high}, learning $f_\theta$ remains well-conditioned because $c^{\mathrm{low}}$ is minimally corrupted. In contrast to monolithic regression, we can train $g_\phi$ on a residual target in coefficient space,
\begin{equation}
\tilde r^{\mathrm{high}} := \tilde c^{\mathrm{high}} - \mathbb{E}[\tilde c^{\mathrm{high}} \mid o, c^{\mathrm{low}}],
\end{equation}
so the model focuses on the predictable, task-conditioned part of high-frequency behavior rather than fitting demonstration-specific noise. Consequently, our factorization is most beneficial on tasks whose success requires reliable high-frequency corrections (precision alignment and rapid impact), and it degrades gracefully when demonstrations are noisy.


\subsection{Learning Formulation}

\subsection{Inference and Execution}


\subsection{problem statement comment}

To reason about temporal structure, we operate on short action segments rather than individual timesteps. Given a sequence of actions, we define a length-$K$ action chunk
\[
a_{t:t+K-1} = (a_t, \ldots, a_{t+K-1}) \in \mathbb{R}^{K \times d}.
\]

We represent each action chunk in a temporal frequency domain using the discrete cosine transform (DCT), which expresses a discrete signal as a weighted sum of cosine basis functions. For a temporal signal $x \in \mathbb{R}^K$, the DCT is defined as
\[
c_k = \sum_{n=0}^{K-1} x_n 
\cos\!\left(\frac{\pi}{K}\left(n+\tfrac{1}{2}\right)k\right),
\qquad k = 0,\ldots,K-1.
\]

Applying this transform independently to each action dimension yields
\[
c_t = F a_{t:t+K-1},
\qquad
a_{t:t+K-1} = F^{-1} c_t,
\]
where $F$ denotes the corresponding orthonormal DCT matrix.

In this representation, low-frequency coefficients capture slowly varying motion, while high-frequency coefficients capture rapid temporal changes, providing a simple and interpretable view of action behavior across temporal scales.




\subsection{old method overview}

We model robotic action generation as a coarse-to-fine process over temporal scales.
Given a short action chunk $a_{t:t+t'}$, we first transform the sequence into a temporal frequency domain using the discrete cosine transform (DCT), and decompose it into low- and high-frequency components.
The action can be written as
\[
a_{t:t+t'}
=
a^{\mathrm{low}}_{t:t+t'}
+
a^{\mathrm{high}}_{t:t+t'},
\]
where the low-frequency component captures smooth, slowly varying motion that determines task-level progress, while the high-frequency component captures short-timescale variations related to precise alignment and contact.

Based on this representation, we impose a causal structure on action generation.
The low-frequency component is predicted from the observation and language instruction,
\[
a^{\mathrm{low}} \sim \pi^{\mathrm{low}}_\theta(o_t, l),
\]
while the high-frequency component is predicted conditionally on the realized coarse motion,
\[
a^{\mathrm{high}} \sim \pi^{\mathrm{high}}_\theta(o_t, a^{\mathrm{low}}).
\]
This factorization separates task-level intent from execution-level refinement, enabling more stable learning of fine-grained actions under noisy demonstrations.

==> tables/ablation.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccccc}
\toprule
Dataset & Stack & Coffee & Libero10 & \multicolumn{3}{c}{Libero-90 (Set A)} & \multicolumn{3}{c}{Libero-90 (Set B)} \\
Noise Injection &  &  &  & No & Small & Large & No & Small & Large \\
\midrule
Frequency Diffusion & \textbf{81.3} & 56.3 & 61.3 & 92.5 & 78.5 & 73.0 & 94.0 & 77.5 & 63.8 \\
No Hierarchy & 73.8 & 77.5 & 56.3 & 95.5 & 85.5 & 81.5 & \textbf{96.0} & 81.5 & 72.5 \\
\textbf{CSP} & 75.0 & \textbf{82.5} & \textbf{74.0} & \textbf{97.0} & \textbf{92.0} & \textbf{87.5} & 94.0 & \textbf{84.0} & \textbf{80.0} \\

\bottomrule
\end{tabular}
\vspace{2pt}
\caption{\textbf{Ablation Study.}}
\label{tab:ablation}
\end{table*}


==> tables/fig5-tableversion.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption*{\textbf{Sensitivity to Low-High Frequency Split.}}
\label{tab:rebuttal_ablation}
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \textbf{Libero-90} & \textbf{Libero-10} & \textbf{Stack} & \textbf{Coffee} \\
\midrule
2 & 89.0 & 73.5 & 86.2 & 83.5 \\
4 & 88.9 & 75.0 & 87.5 & 84.0 \\
6 & 90.8 & 79.0 & 88.3 & 82.0 \\
8 & 90.7 &	77.5 &	87.8 &	83.0 \\
10 &	91.8 &	79.0 &	88.0 &	83.5 \\
12 &	91.6 &	77.0 &	87.6 &	81.0 \\
14 &	90.5 &	75.5 &	87.4 &	79.5 \\
16 &	90.1 &	76.0 &	87.2 &	80.0 \\
18 &	89.8 &	74.5 &	86.0 &	77.5 \\
20 &	88.7 &	77.0 &	85.2 &	79.0 \\
22 &	86.7 &	73.5 &	84.5 &	75.5 \\
24 &	88.1 &	72.5 &	83.2 &	72.0 \\
26 &	85.7 &	71.5 &	81.0 &	75.5 \\
28 &	85.4 &	72.5 &	78.0 &	61.0 \\
30 &	85.7 &	72.0 &	74.0 &	52.0 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/noise.tex <==
\begin{table*}[t]
\centering
\small
\caption{\textbf{Robustness to Demonstration Noise.}
Success rate (in \%) under three dataset conditions: \textbf{No Noise}, \textbf{Low Noise}, and \textbf{High Noise}.
Values are reported as integers for clarity. Missing entries are marked as ``--''.}
\label{tab:noise}
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lccc ccc ccc ccc ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{\textbf{Task-1}} 
& \multicolumn{3}{c}{\textbf{Task-2}} 
& \multicolumn{3}{c}{\textbf{Task-3}} 
& \multicolumn{3}{c}{\textbf{Task-4}} 
& \multicolumn{3}{c}{\textbf{Task-5}} 
& \multicolumn{3}{c}{\textbf{Libero-90 (Set A)}} 
& \multicolumn{3}{c}{\textbf{Libero-90 (Set B)}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}
\textbf{Method}
& \textbf{No} & \textbf{Low} & \textbf{High}
& \textbf{No} & \textbf{Low} & \textbf{High}
& \textbf{No} & \textbf{Low} & \textbf{High}
& \textbf{No} & \textbf{Low} & \textbf{High}
& \textbf{No} & \textbf{Low} & \textbf{High}
& \textbf{No} & \textbf{Low} & \textbf{High}
& \textbf{No} & \textbf{Low} & \textbf{High} \\
\midrule

ACT
& 85 & 70 & 15
& 90 & 80 & 65
& 90 & 80 & 80
& -- & -- & --
& -- & -- & --
& -- & -- & --
& -- & -- & -- \\

DP-CNN
& 90 & 80 & 15
& 100 & 90 & 80
& 95 & 90 & 30
& 95 & 75 & 15
& 90 & 70 & 40
& -- & -- & --
& -- & -- & -- \\

BAKU
& 95 & 80 & 20
& 90 & 80 & 70
& 100 & 60 & 45
& 95 & 80 & 0
& 90 & 70 & 10
& -- & -- & --
& -- & -- & -- \\

Action Binning
& 100 & 50 & 0
& 95 & 80 & 80
& 90 & 70 & 55
& 100 & 80 & 30
& 100 & 85 & 50
& -- & -- & --
& -- & -- & -- \\

Freq-Autoregressive
& 95 & 65 & 10
& 100 & 90 & 70
& 95 & 75 & 55
& 95 & 75 & 35
& 100 & 70 & 45
& -- & -- & --
& -- & -- & -- \\

\textbf{Ours}
& \textbf{90} & \textbf{100} & \textbf{55}
& \textbf{95} & \textbf{100} & \textbf{95}
& \textbf{100} & \textbf{90} & \textbf{85}
& \textbf{90} & \textbf{80} & \textbf{45}
& \textbf{95} & \textbf{85} & \textbf{80}
& -- & -- & --
& -- & -- & -- \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/rebuttal-ablations.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption*{\textbf{Additional Ablations.}}
\label{tab:rebuttal_ablation}
\begin{tabular}{llcccc}
\toprule
\textbf{Low-Freq Condition} & \textbf{High-Freq Condition} & \textbf{Libero-90 (K=16)} & \textbf{Libero-90 (K=32)} & \textbf{Libero-10 (K=16)} & \textbf{Libero-10 (K=32)} \\
\midrule
obs & lang + obs + low-freq & 22.2 & 18.2 & 64.5 & 61.0 \\
lang + obs & low-freq & 74.3 & 69.9 & 68.5 & 66.5 \\
lang + obs & obs & 86.2 & 84.2 & 65.0 & 51.5 \\
lang + obs & low-freq + lang & 91.6 & 90.4 & 81.0 & 75.0 \\
high-freq + obs & lang + obs (predict high-freq first) & 49.6 & 46.0 & 35.5 & 55.5 \\
high-freq + lang + obs & lang + obs (predict high-freq first) & 80.33 & 66.8 & 49.5 & 46.0 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/teleop-kl-divergence.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption*{\textbf{Collection Method KL Divergence.}}
\label{tab:teleop_divergence}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Task} & \textbf{Action KL} & \textbf{Action KL} & \textbf{Freq KL W16} & \textbf{Freq KL W16} & \textbf{Freq KL W32} & \textbf{Freq KL W32} & \textbf{Freq KL W64 } & \textbf{Freq KL W64} \\
& (Orig vs Teleop) & (Syn vs Teleop) & (Orig vs Teleop) & (Syn vs Teleop) & (Orig vs Teleop) & (Syn vs Teleop) & (Orig vs Teleop)& (Syn vs Teleop) \\
\midrule
KITCHEN SCENE 10 Close drawer & 11.71 & 8.42 & 0.71 & 0.55 & 0.74 & 0.60 & 1.06 & 0.82 \\
LIVING ROOM 1 Pick cream cheese & 9.59 & 7.12 & 0.58 & 0.47 & 0.69 & 0.55 & 0.95 & 0.73 \\
LIVING ROOM 5 Mug on plate (yellow) & 10.28 & 7.85 & 0.50 & 0.42 & 0.65 & 0.52 & 0.85 & 0.69 \\
LIVING ROOM 6 Mug on plate (white) & 10.27 & 7.91 & 0.63 & 0.51 & 0.72 & 0.58 & 0.93 & 0.74 \\
STUDY 1 Pick book & 10.99 & 8.36 & 0.65 & 0.54 & 0.70 & 0.59 & 0.91 & 0.76 \\
\textbf{Mean} & 10.57 & 7.93 & 0.61 & 0.50 & 0.70 & 0.57 & 0.94 & 0.75 \\
\bottomrule
\end{tabular}
\end{table}
